Multimodal Auto Validation For Self-Refinement in Web Agents

As our world digitizes, web agents that can automate complex and monotonous tasks are becoming essential in streamlining workflows. This paper introduces an approach to improving web agent performance through multi-modal validation and self-refinement. We present a comprehensive study of different modalities (text, vision) and the effect of hierarchy for the automatic validation of web agents, building upon the state-of-the-art Agent-E web automation framework. We also introduce a self-refinement mechanism for web automation, using the developed auto-validator, that enables web agents to detect and self-correct workflow failures. Our results show significant gains on Agent-E's (a SOTA web agent) prior state-of-art performance, boosting task-completion rates from 76.2\% to 81.24\% on the subset of the WebVoyager benchmark. The approach presented in this paper paves the way for more reliable digital assistants in complex, real-world scenarios.

==> sections/evaluation.tex <==
\section{How to evaluate LLM (agents)?}
Ideally, we would like agents to be improved by themselves from external signals. Realistically, agents are often not able to evaluate reward signals for a given environment. This is an open research problem in itself.

Below are settings that contain feedback for evaluation purposes:

\begin{itemize}
    \item Simulations/Open-world Environments:
    \begin{itemize}
        \item MLAgentBench: coding solutions to ML problems 
        \item AgentBench: operating system (OS), database (DB), knowledge graph (KG), digital card game (DCG), lateral thinking puzzles (LTP), house-holding (Alfworld)\textsuperscript{[1]}, web shopping (WebShop)\textsuperscript{[2]}, and web browsing (Mind2Web)
        \item Minecraft
        \item \textbf{Issue:} Signal of reward is only given after a trajectory roll-out.
    \end{itemize}

    \item Datasets:
    \begin{itemize}
    \item ToolBench: This is a dataset for instruction tuning for +16,000 APIs. For some generated instruction (for a specific API call(s)), a DFS is done over all possible sequences of API calls until the task is completed or not completed (or took too long). Refer to Section 2.2 for more details.
    \item EasyTool
    \item Reasoning settings: Arithmetic, Commonsense, Logic, Symbolic 
    \item \textbf{Benefit:} Dataset already contains (good) trajectory roll-outs.
    \end{itemize}
\end{itemize}



==> sections/lit_review.tex <==
\section{Literature Review}

\subsection{Prompting and Reasoning}
Chain-of-though reasoning [Wei et al 2022] \\
Zero-Shot Reasoners [Kojima et al 2022] \\
Self-Consistency Improves Chain of Thought Reasoning in Language Models [Wang et al 2023] \\
Is ChatGPT a General-Purpose Natural Language Processing Task Solver? [Qin et al 2023] \\
 A Survey of Chain of Thought Reasoning [Chu et al 2023] \\
 Tree of Thought: Deliberate Problem Solving with Large Language Models [Yao et al 2023]\\

\subsection{Self-Improvement}
Think Before You Speak \\
Parsel \\
Quiet-STAR/Self-Taught Reasoner \\
Fun Search \\



\subsection{Uncertainty Aware LLMs}
Teaching models to express their uncertainty in words [Lin et al 2022] \\
Robots That Ask For Help: Uncertainty Alignment for Large Language Model Planners 
[Ren et al 2023] \\
Language Models (Mostly) Know What They Know [Anthropic 2022] \\

\subsection{LLM Agents}

\subsection{Planning}


\section{Open Directions}

